Open source models for the parametric study of diffraction gratings in 2D/2.5D/3D with ONELAB/Gmsh/GetDP

This document aims at presenting both theoretical and practical aspects of the grating2D.pro and grating3D.pro [1] ONELAB [2] models. The 2D model grating2D.pro applies to so-called mono-dimensional gratings, i.e. structures having one direction of invariance. Various geometries and materials can be handled or easily added. The two classical scalar polarization cases, denoted here E// and H//, are addressed as well as the conical vector case. The output consists in a full energy balance of the problem computed from the field maps. The 3D vector model grating3D.pro applies to crossed-gratings. These models are based on free the open source software Gmsh, GetDP and their interface ONELAB. [1] https://gitlab.onelab.info/doc/models/-/wikis/Diffraction-gratings [2] https://onelab.info

==> chap3D.tex <==
\chapter[\tt grating3D.pro]{Crossed gratings : {\tt grating3D.pro}}
\section{Intro}
We denote by $\x$, $\y$ and $\z$ the unit vectors of the axes of an
orthogonal coordinate system $Oxyz$. We only deal with time-harmonic
fields; consequently, electric and magnetic fields are represented
by the complex vector fields $\bE$ and $\bH$, with a time dependance
in $\exp(-i\, \omega\, t)$. Note that incident light is now propagating 
along the $z$-axis, whereas $y$-axis was used in the 2D case. 

Besides, in this section, for the sake of simplicity, the materials are assumed to be isotropic and therefore are optically characterized by their relative permittivity $\varepsilon$ and relative permeability $\mu$. It is of importance to note that lossy materials can be studied, the relative permittivity and relative permeability being represented by complex valued functions. The crossed-gratings we are dealing with  can be split into the following regions:
\begin{itemize} 
	\item%
		\textit{The  superstrate} ($z> z_0$) is
		supposed to be homogeneous, isotropic and lossless, and therefore characterized
		by its relative permittivity $\varepsilon_r^+$ and its relative
		permeability
		$\mu_r^+$ and we denote $k^+:=k_0\, \sqrt{\varepsilon_r^+ \mu_r^+}$, where $k_0:=\omega/c$,%
	\item%
		\textit{The multilayered stack} ($z_N<z<z_0$) is made of $N$ layers which are supposed to be
		homogeneous and isotropic, and therefore characterized by their relative permittivity
		$\varepsilon_r^n$, their relative permeability
		$\mu_r^n$ and their thickness $e_n$. We denote
		$k_n:=~k_0\,\sqrt{\varepsilon_r^n\,\mu_r^n}$ for $n$ integer between $1$ and $N$.
	\item
		\textit{The groove region} ($z_{g}<z<z_{g-1}$), which is embedded in
		the layer indexed $g$ $(\varepsilon_r^g,\mu_r^g)$ of the previously
		described domain, is heterogeneous. Moreover
		the method does work irrespective of whether the
		diffractive elements are homogeneous: The permittivity and permeability can
		vary continuously (gradient index gratings) or discontinuously (step
		index gratings). This region is thus characterized by the
		scalar fields $\varepsilon_r^{g'}(x,y,z)$ and $\mu_r^{g'}(x,y,z)$. The
		groove periodicity along the $x$--axis, respectively (resp.) $y$--axis, is denoted
		$d_x$, resp. $d_y$, in the sequel.
	\item%
		\textit{The substrate} ($z<z_N$) is supposed to be homogeneous
		and isotropic and therefore characterized by its relative
		permittivity $\varepsilon_r^-$ and its relative permeability
		$\mu_r^-$ and we denote $k^-:=k_0\, \sqrt{\varepsilon_r^- \mu_r^-}$,%
	\end{itemize}
	The incident field on this structure is denoted:
	\begin{equation}\label{eq:def_Einc}
		\bE^{\mathrm{inc}} =\textbf{A}_0^e\;\textrm{exp}(i \,\textbf{k}^+\cdot\textbf{r})
	\end{equation}
	with
	\begin{equation}\label{eq:def_kplus}
		\textbf{k}^+ = \left[ \begin{array}{l} \alpha_0\\\beta_0\\\gamma_0
		\end{array} \right] = k^+\,\left[ \begin{array}{l} -\sin \theta_0 \,\cos \varphi_0 \\-\sin \theta_0 \,\sin \varphi_0 \\-\cos \theta_0
		\end{array} \right]
	\end{equation}
	and
	\begin{equation}\label{eq:def_Azero}
		\textbf{A}_0^e = \left[ \begin{array}{l} E^0_x\\E^0_y\\E^0_z
		\end{array} \right] =A^e\,\left[ \begin{array}{l} \cos \psi_0 \, \cos \theta_0  \,\cos \varphi_0  - \sin \psi_0 \, \sin \varphi_0 \\\cos \psi_0 \, \cos \theta_0 \, \sin \varphi_0  + \sin \psi_0 \, \cos \varphi_0 \\-\cos \psi_0 \, \sin \theta_0
		\end{array} \right] ,
	\end{equation}
	where $\varphi_0\in[0,2\pi]$, $\theta_0\in[0,\pi/2]$ and
	$\psi_0\in[0,\pi]$ (polarization angle).
	
	We recall here the diffraction problem: finding the solution of Maxwell equations in harmonic
	regime \textit{i.e.} the unique solution ($\bE,\bH$) of:
	\begin{subequations}\label{eq:Maxwell2}
		\begin{numcases}{}
			\curl\, \bE=i \omega \mu_0\, \tensmur \, \bH \label{eq:MaxwellrotE2}\\
			\curl\, \bH=-i \omega \varepsilon_0\, \tensepsr \, \bE
			\label{eq:MaxwellrotH2}
		\end{numcases}
	\end{subequations}
	such that the diffracted field satisfies the so-called
	\textit{Outgoing Waves Condition} (OWC) and
	where $\bE$ and $\bH$ are quasi-bi-periodic functions with respect
	to $x$ and $y$ coordinates.
	
\section{Notations}
One can choose to calculate arbitrarily $\bE$, since $\bH$ can be
deduced from Eq.~(\ref{eq:MaxwellrotE2}). The diffraction problem
amounts to looking for the unique solution $\bE$ of the so-called
vectorial Helmholtz propagation equation, deduced from
Eqs.~(\ref{eq:MaxwellrotE2},\ref{eq:MaxwellrotH2}):
\begin{equation}\label{eq:defLvect}
    \Lvect_{\varepsilon,\nucol}:=-\curl\left(\tensnur\,\curl\bE\right) + k_0^2\,\tensepsr\,\bE =
    \textbf{0}
\end{equation} 
such that the diffracted field satisfies an OWC and where $\bE$ is a quasi-bi-periodic function with respect to $x$ and $y$ coordinates. 

\subsubsection{From a diffraction problem to a radiative one with  localized sources}\label{part:radiation_pb}
As depicted in Fig.~\ref{fig:schema_3D_multi}, the scalar relative permittivity $\tensepsr$ and {inverse} permeability $\tensnur$ tensor fields associated to the studied diffractive structure can be written using complex-valued functions defined by part and taking into account the notations adopted in Sec.~\ref{part:3D_def_notations}. We will consider isotropic materials ($\tensepsr=\varepsilon_r\,\tensid$ and $\tensnur=\nu_r\,\tensid$) for the structure but it is worth keeping the tensor notations in mind because we are going to use PMLs.
\begin{equation}\label{eq:def_eps_global}
\upsilon(x,y,z):= \left \{
\begin{array}{lcccc}
  \upsilon^+ & \hbox{for} & z>z_0 &&\\
  \upsilon^n & \hbox{for} & z_{n-1}>z>z_n & \hbox{with} & 1\leq n < g\\
  \upsilon^{g'}(x,y,z) & \hbox{for} & z_{g-1}>z>z_g &&\\
  \upsilon^n & \hbox{for} & z_{n-1}>z>z_n& \hbox{with} & g<n \leq N\\
  \upsilon^- & \hbox{for} & z<z_N&&
\end{array}
\right .
\end{equation}
\noindent with $\upsilon=\{ \varepsilon, \nucol \}\quad , \quad
z_0=0 \quad \textrm{and} \quad z_n = -\sum_{l=1}^{n}e_l \quad
\textrm{for} \quad 1\leq n \leq N$.

\noindent It is now convenient to introduce two functions defined by
part $\varepsilon_1$ and $\nucol_1$ corresponding to the associated
multilayered case (\textit{i.e.} the same stack without any
diffractive element) constant over $Ox$ and $Oy$:
\begin{equation}\label{eq:def_eps1}
\upsilon_1(x,y,z):= \left \{
\begin{array}{lcccc}
  \upsilon^+ & \hbox{for} & z>0\\
  \upsilon^n & \hbox{for} & z_{n-1}>z>z_n & \hbox{with} & 1\leq n \leq N\\
  \upsilon^- & \hbox{for} & z<z_N
\end{array}
\right .
\end{equation}
\noindent with $\upsilon=\{ \varepsilon, \nucol \}$.

\noindent We denote by $\bE_0$ the restriction of
$\bE^{\mathrm{inc}}$ to the superstrate region:
\begin{equation}
\bE_0:= \left \{
\begin{array}{ccc}
  \bE^{\mathrm{inc}} & \hbox{for} & z>z_0 \\
  \mathbf{0} & \hbox{for} & z\leq z_0
\end{array}
\right .%
\end{equation}
\noindent We are now in a position to define more explicitly the
vector diffraction problem that we are dealing with in this
section. It amounts to looking for the unique vector field $\bE$
solution of:
\begin{equation}\label{eq:defLOWC_vect}
    \Lvect_{\varepsilon,\nucol}(\bE)=\mathbf{0} \quad \hbox{such that $\bE^d:=\bE-\bE_0$
satisfies an OWC.}
\end{equation}
\noindent In order to reduce this diffraction problem to a radiation
one {\emph with bounded sources}, an intermediary vector field denoted $\bE_1$ is necessary and
is defined as the unique solution of:
\begin{equation}\label{eq:defL1_vect}
    \Lvect_{\varepsilon_1,\nucol_1}(\bE_1)=\mathbf{0} \quad \hbox{such that $\bE_1^d:=\bE_1-\bE_0$ satisfies an OWC.}
\end{equation}
\noindent The vector field $\bE_1$ corresponds to an \textit{ancillary
problem} associated to the \textit{general vectorial case of a
multilayered stack} which can be calculated \textit{independently}.
This general calculation is seldom treated in the literature, we
present a development in Appendix. Thus $\bE_1$ is from now on
\textit{considered as a known} vector field. It is now apropos to
introduce the unknown vector field $\bE_2^d$, simply defined as the
difference between $\bE$ and $\bE_1$, which can finally be
calculated thanks to the FEM and:
\begin{equation}\label{eq:E2d}
\bE_2^d:= \bE - \bE_1 =\bE^d-\bE_1^d\; .
\end{equation}
It is of importance to note that the presence of the superscript $d$
is not fortuitous: As a difference between two diffracted fields
(Eq.~(\ref{eq:E2d}), $\bE_2^d$ satisfies an OWC which is of prime
importance in our formulation. By taking into account these new
definitions, Eq.~(\ref{eq:defLOWC_vect}) can be written:
\begin{equation}\label{eq:radiating_vect}
    \Lvect_{\varepsilon,\nucol}(\bE_2^d) = -\Lvect_{\varepsilon,\nucol}(\bE_1)
\; ,
\end{equation}
\noindent where the right-hand member is a vector field which can be
interpreted as \textit{a known vectorial source term
$-\Svect_1(x,y,z)$ whose support is localized inside the diffractive
element itself}. To prove it, let us introduce the null term defined
in Eq.~(\ref{eq:defL1_vect}) and make the use of the linearity of
$\Lvect$, which leads to:
\begin{equation}
    \Svect_1:=\Lvect_{\varepsilon,
    \nucol}(\bE_1)=\Lvect_{\varepsilon,
    \nucol}(\bE_1)-\underbrace{\Lvect_{\varepsilon_1,
    \nucol_1}(\bE_1)}_{=\mathbf{0}}=\Lvect_{\varepsilon-\varepsilon_1, \nucol -
    \nucol_1}(\bE_1) \; .
\end{equation}
\begin{figure}[t]
	\centering
	\includegraphics[width=.4\textwidth]{figs3D/angles.pdf}
	\caption{Angles convention for the incident plane wave.}
	\label{fig:conv}
\end{figure}


\section{Quasi-periodicity and weak formulation}\label{part:form_faible_3D}
The weak form residue is obtained by multiplying scalarly
Eq.~(\ref{eq:defLOWC_vect}) by weighted vectors $\bE'$ chosen among
the ensemble of quasi-bi-periodic vector fields of $H^1(\Omega,\curl)$
(denoted $H^1\left(\Omega,\curl,(d_x,d_y),\bk\right)$) :
\begin{equation}\label{eq:R_vect_def}
    \Rvect_{\varepsilon,\nucol}(\bE,\bE')=\int_\Omega -\curl\left(\nucol\,\curl\bE\right)\cdot\overline{\bE'} + k_0^2\,\tensepsr\,\bE\cdot\overline{\bE'}\,\mathrm{d}\Omega
\end{equation}
\noindent Integrating by part Eq.~(\ref{eq:R_vect_def}) and making
the use of the Green-Ostrogradsky theorem lead to:
\begin{equation}\label{eq:weak}
    \Rvect_{\varepsilon,\nucol}(\bE,\bE')=\int_\Omega -\nucol\,\curl\bE\cdot\curl\overline{\bE'} +
    k_0^2\,\varepsilon\,\bE\cdot\overline{\bE'}\,\mathrm{d}\Omega -
    \int_{\partial \Omega}\left(\n \times (\nucol\,\curl\bE)\right)\cdot\overline{\bE'}\,\mathrm{d}S
\end{equation}
where $\n$ refers to the exterior unit vector normal to the surface
$\partial \Omega$ enclosing $\Omega$.

\section{Template examples}
The test cases provided below will help understanding the possibilities offered by this model.
\subsection{Bi-sinusoidal}
\subsection{Checkerboard}
\subsection{Half-ellipsoid}
\subsection{Hole in metal plate}
\subsection{Pyramid}
\subsection{Torus}
\subsection{Fake 2D conical}
\subsection{Solar cell}
\subsection{Convergence and curved elements}
\subsection{Skew lattice}


==> figs_chap1/test.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=3 by 2}]
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.5,0.5)},
  anchor=center,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={N / mesh size \(\displaystyle \approx\lambda_0/(N\sqrt{\varepsilon_r})\)},
xmin=0.3, xmax=15.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle T^{(N)}_{0,0}\)},
ymin=0.4925876033576, ymax=0.6681822701524,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
1 0.659943342208862
2 0.557811260223389
3 0.53715705871582
4 0.525018453598022
5 0.519052267074585
6 0.518084764480591
7 0.51706326007843
8 0.515566110610962
9 0.512928485870361
10 0.509334325790405
11 0.508147597312927
12 0.506891965866089
13 0.506368517875671
14 0.505754113197327
15 0.505462050437927
};
\addlegendentry{first formula - order 1}
\addplot [semithick, darkorange25512714]
table {%
1 0.636322975158691
2 0.533577680587769
3 0.51711106300354
4 0.507892847061157
5 0.504426002502441
6 0.50474739074707
7 0.503153562545776
8 0.502991676330566
9 0.502140760421753
10 0.501812934875488
11 0.501323103904724
12 0.501223564147949
13 0.500909566879272
14 0.500758767127991
15 0.500569105148315
};
\addlegendentry{first formula - order 2}
\addplot [semithick, forestgreen4416044]
table {%
1 0.660200715065002
2 0.559392929077148
3 0.539116859436035
4 0.525407314300537
5 0.519944310188293
6 0.518606901168823
7 0.517707586288452
8 0.516496658325195
9 0.513530731201172
10 0.509746074676514
11 0.508567929267883
12 0.507744431495667
13 0.506606578826904
14 0.506205081939697
15 0.505914211273193
};
\addlegendentry{second formula - order 1}
\addplot [semithick, crimson2143940]
table {%
1 0.637131452560425
2 0.534881830215454
3 0.518828511238098
4 0.508222103118896
5 0.505060195922852
6 0.505252599716187
7 0.503721475601196
8 0.503984212875366
9 0.50274121761322
10 0.502164840698242
11 0.501723051071167
12 0.502098560333252
13 0.501159071922302
14 0.501199245452881
15 0.501009225845337
};
\addlegendentry{second formula - order 2}
\draw (axis cs:0.06,0.04) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{(a)};

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle N\)},
xmin=0.35, xmax=14.65,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle \frac{|T^{(N)}_{0,0}-T^{(\mathrm{ref})}_{0,0}|}{T^{(\mathrm{ref})}_{0,0}}\)},
ymin=0.000270578163938772, ymax=0.441316527360715,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black, dashed, mark=|, mark size=3, mark options={solid}]
table {%
1 0.315303981304169
2 0.113246940076351
3 0.0723848417401314
4 0.0483699813485146
5 0.0365666225552559
6 0.0346525795757771
7 0.032631628215313
8 0.0296698473393917
9 0.0244515836238861
10 0.0173408277332783
11 0.014993098564446
12 0.0125089138746262
13 0.0114733250811696
14 0.0102578438818455
};
\addlegendentry{order 1}
\addplot [semithick, black, mark=|, mark size=3, mark options={solid}]
table {%
1 0.271198779344559
2 0.0659419447183609
3 0.0330463014543056
4 0.0146306473761797
5 0.00770475855097175
6 0.00834692362695932
7 0.00516290310770273
8 0.00483957072719932
9 0.00313945533707738
10 0.00248470669612288
11 0.00150615291204304
12 0.00130722380708903
13 0.000680126366205513
14 0.000378715951228514
};
\addlegendentry{order 2}
\draw (axis cs:0.03,0.04) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{(b)};

\nextgroupplot[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle N\)},
xmin=0.3, xmax=15.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Number of unkowns},
ymin=437.309203489468, ymax=294944.435129197,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black, dashed, mark=|, mark size=3, mark options={solid}]
table {%
1 587.999877929688
2 1837.99963378906
3 2784
4 4582
5 6716.00146484375
6 9869.998046875
7 12290.0009765625
8 17149.990234375
9 22023.98828125
10 27746.013671875
11 33568.01171875
12 42583.98046875
13 49944.015625
14 62291.984375
15 70912.03125
};
\addplot [semithick, black, mark=|, mark size=3, mark options={solid}]
table {%
1 1607.99963378906
2 5198.9990234375
3 8060.00146484375
4 13344.998046875
5 19865
6 29399.013671875
7 36839.98828125
8 51762.015625
9 66916.96875
10 84438.0078125
11 102553.96875
12 130423.96875
13 153472.9375
14 192395.9375
15 219357.109375
};
\draw (axis cs:0.06,0.9) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{(c)};

\nextgroupplot[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle N\)},
xmin=0.3, xmax=15.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={MUMPs wall time (s)},
ymin=0.280795598889986, ymax=54.5072308686596,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black, dashed, mark=|, mark size=3, mark options={solid}]
table {%
1 0.356774002313614
2 0.500698983669281
3 0.63979297876358
4 0.833141088485718
5 1.15260004997253
6 1.57997989654541
7 1.93166029453278
8 2.7471604347229
9 3.35821032524109
10 4.29383087158203
11 5.279541015625
12 6.8545994758606
13 8.2496223449707
14 10.4231004714966
15 12.4277000427246
};
\addplot [semithick, black, mark=|, mark size=3, mark options={solid}]
table {%
1 0.417949020862579
2 0.740162074565887
3 0.993670880794525
4 1.55080986022949
5 2.28111982345581
6 3.19232082366943
7 4.27041006088257
8 6.42151069641113
9 8.81008148193359
10 11.9724016189575
11 14.9020013809204
12 20.6609992980957
13 24.8067016601562
14 35.8668975830078
15 42.8993949890137
};
\draw (axis cs:0.06,0.9) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{(d)};

\nextgroupplot[
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle N\)},
xmin=0.3, xmax=15.7,
xtick style={color=black},
y grid style={darkgray176},
ylabel={RAM allocated (Mb)},
ymin=31.632029794774, ymax=10835.5720875879,
ymode=log,
ytick style={color=black}
]
\addplot [semithick, black, dashed, mark=|, mark size=3, mark options={solid}]
table {%
1 41.2421951293945
2 63.2539100646973
3 82.6952972412109
4 114.104988098145
5 159.852035522461
6 218.945053100586
7 273.624969482422
8 389.902038574219
9 503.988037109375
10 661.613098144531
11 818.64111328125
12 1076.59008789062
13 1312.42980957031
14 1641.94995117188
15 2013.67956542969
};
\addplot [semithick, black, mark=|, mark size=3, mark options={solid}]
table {%
1 59.8945121765137
2 131.387008666992
3 187.128952026367
4 305.605102539062
5 475.452972412109
6 727.288940429688
7 912.094055175781
8 1428.2099609375
9 1929.20959472656
10 2587.35986328125
11 3161.84033203125
12 4436.099609375
13 5197.08984375
14 7086.109375
15 8310.6923828125
};
\draw (axis cs:0.06,0.9) node[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{(e)};
\end{groupplot}

\end{tikzpicture}

